Group-blind optimal transport to group parity and its constrained variants

Fairness holds a pivotal role in the realm of machine learning, particularly when it comes to addressing groups categorised by protected attributes, e.g., gender, race. Prevailing algorithms in fair learning predominantly hinge on accessibility or estimations of these protected attributes, at least in the training process. We design a single group-blind projection map that aligns the feature distributions of both groups in the source data, achieving (demographic) group parity, without requiring values of the protected attribute for individual samples in the computation of the map, as well as its use. Instead, our approach utilises the feature distributions of the privileged and unprivileged groups in a boarder population and the essential assumption that the source data are unbiased representation of the population. We present numerical results on synthetic data and real data.

==> arxiv.tex <==


\paragraph{Feasibility:}(not finished)
Theorem~\ref{pro:binary_condition} has transformed the total repair property into a constraint imposed on the coupling $\gamma$. 
Recall the definition of couplings in Equation~\eqref{equ:Pi-define}. A  feasible coupling $\gamma\in\Pi(P^X,P^{\td{X}})$ needs to satisfy $\gamma_{i,j}\geq 0$ for all $i\in\supp{X},j\in\supp{\td{X}}$ and the following
\begin{equation}
\sum_{j\in\supp{\td{X}}}\gamma_{i,j}=P^{X}_i,\forall i\in\supp{X};\quad \sum_{i\in\supp{X}}\gamma_{i,j}=P^{\td{X}}_j, \forall j\in\supp{\td{X}}.\label{equ:coupling-requirement}
\end{equation}
In general, the constraint in Theorem~\ref{pro:binary_condition} and Equation~\eqref{equ:coupling-requirement} could conflict with each other. Below, we give an example.

For example, given an index $i\in\supp{X}$. Let the portions of both groups be $\p{S=s_0}=1e^{-10},\p{S=s_1}=1-1e^{-10}$, Assume all samples in group $s_0$ have feature $X=i$ while no sample in group $s_1$ have feature $X=i$, such that $P^{X_{s_0}}_i=1,P^{X_{s_1}}_i=0$.
Hence, the portion of samples with feature being $X=i$ among all samples is $P^{X}_i=1e^{-10}$ and the $i^{th}$ entry of vector $V$ becomes $V_i=1/1e^{-10}$. 
%
The constraint in Theorem~\ref{pro:binary_condition} imposes that $\sum_{i\in\supp{X}}\gamma_{i,j}V_i=0,\forall j\in\supp{\td{X}}$. 


\begin{definition}[Couplings]\label{def:couplings}
Let $\gamma\in\Sigma^2_N$ be a matrix (coupling) where its entry is defined to be the joint distribution of $X,\td{X}$, i.e., 
\begin{equation}
\gamma_{i,j}:=\p{X=i,\td{X}=j},
\end{equation}
such that it holds
\begin{equation}
\gamma\mathbb{1}=P^{X},\quad \gamma^{\tr}\mathbb{1}=P^{\td{X}}.
\end{equation}
The set of all admissible couplings $\gamma$ that is able to transport $P^{X}$ to $P^{\td{X}}$, is defined as 
\begin{equation}
\Pi(P^{X},P^{\td{X}}):=\{\gamma\in\Sigma^2_N\mid \gamma\mathbb{1}=P^{X}, \gamma^{\tr}\mathbb{1}=P^{\td{X}}\}.
\end{equation}
\end{definition}

\subsection{A Discussion}
Theorem~\ref{pro:binary_condition} has transformed the total repair property into a constraint imposed on the coupling $\gamma$.
Then, we need to figure out what does such couplings satisfying Theorem~\ref{pro:binary_condition} look like.
Note that $\gamma_{i,j}\geq 0$.
If we set
\begin{align}
\gamma_{i,j}=0,\; \forall i\in\{i\in\supp{X}\mid P^{X_{s_0}}_i\neq P^{X_{s_1}}_i \}, \forall j\in\supp{\td{X}},\label{equ:initial-idea}
\end{align}
we have Equation~\eqref{equ:coupling-condition-binary-simple} satisfied, such that total repair is guaranteed.
However, Definition~\ref{def:couplings} requires that the coupling $\gamma\in\Pi(P^{X},P^{\td{X}})$ should also satisfy 
\begin{equation}
\sum_{j\in\supp{\td{X}}}\gamma_{i,j}=P^{X}_i,\forall i\in\supp{X};\quad \sum_{i\in\supp{X}}\gamma_{i,j}=P^{\td{X}}_j, \forall j\in\supp{\td{X}}.\label{equ:coupling-requirement}
\end{equation}
In general, Equations~\eqref{equ:initial-idea} and \eqref{equ:coupling-requirement} could conflict with each other: 
\begin{itemize}
\item First, for $i\in\{i\in\supp{X}\mid P^{X_{s_0}}_i\neq P^{X_{s_1}}_i\}$, we set $\gamma_{i,j}=0$, for $j\in\supp{\td{X}}$. Then, we have that $\sum_{ j\in\supp{\td{X}}}\gamma_{i,j}$ must be zero, while $P^{X}_i$ is not necessarily zero.
\item Further, when $P^{X_{s_0}}_i\neq P^{X_{s_1}}_i$ for any $i\in\supp{X}$, we have to set $\gamma_{i,j}=0$ everywhere.
In this case, $\sum_{i\in\supp{X}}\gamma_{i,j}$ can only be zero, while $P^{\td{X}}_j$ is not necessarily zero.
\end{itemize}
Due to these potential conflicts, we cannot directly set $\gamma_{i,j}=0$ for any $i$ that $P^{X_{s_0}}_i\neq P^{X_{s_1}}_i$. Instead, we can focus on the non-zero rows in $V$ and try to minimise the entries of $\gamma^{\tr}V$.

\begin{example}\label{exa:col-sparsity}
Let $\supp{X}=\supp{\td{X}}:=\{1,2,3\}$. Suppose $\supp{S}:=\{s_0,s_1\}$ and $P^{S}:=[0.6,0.4]^{\tr}$. Let $P^{X_{s_0}}:=[0.1,0.9,0]^{\tr}$ and $P^{X_{s_1}}:=[0.1,0.4,0.5]^{\tr}$. 
The probability distribution of $X$ is the linear combination in Equation~\eqref{equ:linear-combination-source}, thus $P^{X}=[0.1,0.7,0.2]^{\tr}$.
Now, we calculate
\begin{equation}
V=[0,\;5/7,\;-5/2]^{\tr}
\end{equation}
We set the target distribution of $P^{\td{X}}:=[0.4,0.3,0.3]^{\tr}$. 
Note that $V_2,V_3\neq 0$. 
Let us compare two couplings $\gamma_0,\gamma_1\in\Pi(P^{X},P^{\td{X}})$:
\NiceMatrixOptions{code-for-first-row = \color{blue},
code-for-last-col =\color{green}}
\begin{equation}
\gamma^{\tr}_0=\begin{pNiceArray}{ccc}[first-row,last-row,first-col,last-col,nullify-dots]
& 0.1 & 0.7 & 0.2 & \\
&0.1 & 0.7/3 & 0.2/3&0.4\\
& & 0.7/3 & 0.2/3&0.4\\
& & 0.7/3 & 0.2/3&0.3\\&&&& 
\end{pNiceArray}
,\quad
\gamma^{\tr}_1=\begin{pNiceArray}{ccc}[first-row,last-row,first-col,last-col,nullify-dots]
& 0.1 & 0.7 & 0.2 & \\
& 0.1 & 0.3 & &0.4\\
& & 0.3 & &0.3\\
& & 0.1 & 0.2&0.3\\&&&& 
\end{pNiceArray},
\end{equation}
where the blue texts show $P^{X}$ and the green texts show $P^{\td{X}}$. Note that both couplings are feasible, while the first one $\gamma_0$ has higher sparsity for $i=2,3$. Now ,we can compute the resulted $P^{\td{X_s}}$ from both couplings:
\begin{itemize}
\item Using the coupling $\gamma_0$:
\begin{align*}
P^{\td{X}_{s_0}}=\gamma^{\tr}_0 \frac{P^{X_0}}{P^X} =[0.4,0.3,0.3]^{\tr},\quad
P^{\td{X}_{s_1}}=\gamma^{\tr}_0 \frac{P^{X_1}}{P^X}=[0.4,0.3,0.3]^{\tr}.
\end{align*}
\item Using the coupling $\gamma_1$:
\begin{align*}
P^{\td{X}_{s_0}}=\gamma^{\tr}_1 \frac{P^{X_0}}{P^X} =\frac{1}{70}[34,27,9]^{\tr},\quad
P^{\td{X}_{s_1}}=\gamma^{\tr}_1 \frac{P^{X_1}}{P^X}=\frac{1}{70}[19,12,39]^{\tr}.
\end{align*}

\end{itemize}
In both cases,
Equation~\eqref{equ:linear-combination-target} is satisfied: $P^{\td{X}}=\sum_{s\in\supp{S}}P^{S}_s P^{\td{X}_{s}}$.
But, it is obvious that total repair is satisfied when $\gamma_0$ is used while $\gamma_1$ fails, because
\begin{equation}
\gamma^{\tr}_0 V=\mathbb{0},\quad\gamma^{\tr}_1 V=\frac{3}{14}\times[1,1,-2]^{\tr}.
\end{equation}
\end{example}





\begin{definition}
Let $V\in\bb{R}^{N}$ be a vector
\begin{equation}
V:=\frac{P^{X_{s_0}}-P^{X_{s_1}}}{P^{X}},
\end{equation}
where the subtraction and division operations are element-wise.
\end{definition}

\begin{definition} 
We define the set of indices of non-zero entries in $V$:
\begin{equation} 
\overline{\supp{X}}:=\{i\in\supp{X}\mid V_i\neq 0\}.
\end{equation}
\end{definition}

\begin{lemma}[Fact 2.3 in \cite{bauschke2000dykstras}]\label{lem:Fact 2.3}
Suppose $\varphi$ is Legendre on $E$ and $\mathcal{C}$ is a closed convex set in $E$ with $\mathcal{C}\cap\interior(\dom \varphi)\neq\emptyset$. Let $\xi\in\interior(\dom\varphi)$, then $P^{\varphi}_{\mathcal{C}}(\xi)$ is characterised by
\begin{equation*}
P^{\varphi}_{\mathcal{C}}(\xi)\in\mathcal{C}\cap\interior(\dom \varphi),\quad \langle\nabla\varphi(\xi)-\nabla\varphi\left(P^{\varphi}_{\mathcal{C}}(\xi)\right),c-P^{\varphi}_{\mathcal{C}}(\xi)\rangle\leq 0,\;\forall c\in\mathcal{C}.
\end{equation*}
\end{lemma}

\begin{lemma}[Fact 2.4 in \cite{bauschke2000dykstras}]\label{lem:fact 2.4}
Suppose $\varphi$ is Legendre on $E$. If $\xi,P^{\varphi}_{\mathcal{C}}(\xi)\in\interior(\dom\varphi)$ and $c\in\dom\varphi$, then
\begin{equation*}
D_{\varphi}\left(c,P^{\varphi}_{\mathcal{C}}(\xi)\right)+D_{\varphi}\left(P^{\varphi}_{\mathcal{C}}(\xi),\xi\right)-D_{\varphi}(c,\xi)=
\langle\nabla\varphi(\xi)-\nabla\varphi\left(P^{\varphi}_{\mathcal{C}}(\xi)\right),c-P^{\varphi}_{\mathcal{C}}(\xi)\rangle.
\end{equation*}
\end{lemma}


To solve the optimal transport with inequality constraints, we initialise $\gamma^{(0)}:=\xi=\exp{(-C/\epsilon)}$, 
\begin{equation}
\gamma^{(1)}=\prox^{KL}_{\mathcal{C}_1}(\gamma^{(0)}), \quad\gamma^{(2)}=\prox^{KL}_{\mathcal{C}_2}(\gamma^{(1)}),\quad\gamma^{(3)}=\prox^{KL}_{\mathcal{C}_3}(\gamma^{(2)}),
\end{equation}
then perform the iterations of Dykstra's algorithm: for $n\geq L=3$,
\begin{equation}
\gamma^{(n+1)}=\prox^{KL}_{\mathcal{C}_n}(\gamma^{(n)}\odot q_{n-L+1}), 
\end{equation}
where $\odot$ and $\div$ are element-wise multiplication and division, $\mathcal{C}_n\equiv\mathcal{C}_{1+(n\mod L)}$, and
\begin{equation}
q_{n}:=
\begin{cases}
\frac{\gamma^{(n-1)}}{\gamma^{(n)}}& \textrm{ if }n=1,2,3\\
q_{n-L}\odot\frac{\gamma^{(n-1)}}{\gamma^{(n)}}&\textrm{ otherwise}.
\end{cases}
\end{equation}


\begin{remark}
Let $F(x):=\sum_{i\in\overline{\supp{X}}}\bar{\gamma}_{i,j}V_i\exp{(-V_i x)} + c$, where $c\in\bb{R}$ is a constant. Notice that
\begin{equation}
F'(x)=-\sum_{i\in\overline{\supp{X}}}\bar{\gamma}_{i,j}(V_i)^2\exp{(-V_i x)}\leq 0,
\end{equation}
such that $F(x)$ is a non-increasing function. From Lemma~\ref{lem:prox_c3}, $F(x)=0$ when $x=\nu_j$ if $c=\pm\Theta_j$. The root of function $F(x)$, can be found by Newton-Raphson algorithm, bisection method, Chandrupatla's algorithm, et al..
\end{remark}

for $n>0$
\begin{equation}
\gamma^{(n+1)}=\prox^{KL}_{\mathcal{C}_n} (\gamma^{(n)}), \textrm{ where  }\mathcal{C}_n\equiv\mathcal{C}_{1+(n\mod 2)}.\label{equ:iterative-Bregman-baseline}
\end{equation} 

Introduce one dual variable $\nu\in\bb{R}^N$, the Lagrangian reads:
\begin{equation}
\mathcal{L}(\gamma,\nu)=\kl{\gamma}{\bar{\gamma}}-\nu^{\tr}(\bar{\gamma}^{\tr}V).
\end{equation}
The KKT conditions:
\begin{align}
\frac{\partial \mathcal{L}}{\partial \gamma_{i,j}}=\log\left(\frac{\gamma_{i,j}}{\bar{\gamma}_{i,j}}\right)-V_i\nu_j =0,\\
\nu_j(\sum_{i}\gamma_{i,j}V_i)=0.
\end{align}
The first condition implies $\gamma_{i,j}=\bar{\gamma}_{i,j}\exp{(V_i\nu_j )}$, such that the second condition becomes:
\begin{equation}
\sum_{i}\gamma_{i,j}V_i=\sum_{i}\bar{\gamma}_{i,j}\exp{(\nu_jV_i)}V_i=0.\label{equ:c3-second-condition}
\end{equation}
If $\nu^*_j$ satisfies Equation~\eqref{equ:c3-second-condition}, and $\gamma^*_{i,j}=\bar{\gamma}_{i,j}\exp{(\nu^*_j V_i)}$, then the tuple $(\gamma^*_{i,j},\nu^*_j)$ is optimal, as strong duality holds.



\begin{align*}
\pover{\td{1}}{s_0}&=\sum_{i\in\supp{X_{s_0}}=\{1,2\}}\p{x,\td{1}}\frac{\pover{X=i}{S=s_0}}{\p{X=i}}=0.1\cdot 0.1/0.1+0.7/3\cdot 0.9/0.7=0.4\\
\pover{\td{2}}{s_0}&=\sum_{i\in\supp{X_{s_0}}=\{1,2\}}\p{x,\td{2}}\frac{\pover{X=i}{S=s_0}}{\p{X=i}}=0.7/3\cdot 0.9/0.7=0.3\\
\pover{\td{3}}{s_0}&=\sum_{i\in\supp{X_{s_0}}=\{1,2\}}\p{x,\td{3}}\frac{\pover{X=i}{S=s_0}}{\p{X=i}}=0.7/3\cdot 0.9/0.7=0.3,
\end{align*}
such that $P^{\td{X}_{s_0}}=[0.4,0.3,0.3]^{\tr}$. Similarly, 
\begin{align*}
\pover{\td{1}}{s_1}&=\sum_{i\in\supp{X_{s_1}}=\{1,2,3\}}\p{x,\td{1}}\frac{\pover{X=i}{S=s_1}}{\p{X=i}}=0.1\cdot 0.1/0.1+0.7/3\cdot 0.4/0.7+0.2/3\cdot 0.5/0.2=0.4\\
\pover{\td{2}}{s_1}&=\sum_{i\in\supp{X_{s_1}}=\{1,2,3\}}\p{x,\td{2}}\frac{\pover{X=i}{S=s_1}}{\p{X=i}}=0.7/3\cdot 0.4/0.7+0.2/3\cdot 0.5/0.2=0.3\\
\pover{\td{3}}{s_1}&=\sum_{i\in\supp{X_{s_1}}=\{1,2,3\}}\p{x,\td{3}}\frac{\pover{X=i}{S=s_1}}{\p{X=i}}=0.7/3\cdot 0.4/0.7+0.2/3\cdot 0.5/0.2=0.3,
\end{align*}
such that the probability distribution of $P^{\td{X}_{s_1}}$ is also $[0.4,0.3,0.3]^{\tr}$. 
\item Using the coupling $\gamma_1$:
\begin{align*}
\pover{\td{1}}{s_0}&=\sum_{i\in\supp{X_{s_0}}=\{1,2\}}\p{x,\td{1}}\frac{\pover{X=i}{S=s_0}}{\p{X=i}}=0.1\cdot 0.1/0.1+0.3\cdot 0.9/0.7=17/35\\
\pover{\td{2}}{s_0}&=\sum_{i\in\supp{X_{s_0}}=\{1,2\}}\p{x,\td{2}}\frac{\pover{X=i}{S=s_0}}{\p{X=i}}=0.3\cdot 0.9/0.7=27/70\\
\pover{\td{3}}{s_0}&=\sum_{i\in\supp{X_{s_0}}=\{1,2\}}\p{x,\td{3}}\frac{\pover{X=i}{S=s_0}}{\p{X=i}}=0.1\cdot 0.9/0.7=9/70,
\end{align*}
such that the probability distribution of $P^{\td{X}_{s_0}}=\frac{1}{70}[34,27,9]^{\tr}$. Similarly, 
\begin{align*}
\pover{\td{1}}{s_1}&=\sum_{i\in\supp{X_{s_1}}=\{1,2,3\}}\p{x,\td{1}}\frac{\pover{X=i}{S=s_1}}{\p{X=i}}=0.1\cdot 0.1/0.1+0.3\cdot 0.4/0.7=19/70\\
\pover{\td{2}}{s_1}&=\sum_{i\in\supp{X_{s_1}}=\{1,2,3\}}\p{x,\td{2}}\frac{\pover{X=i}{S=s_1}}{\p{X=i}}=0.3\cdot 0.4/0.7=6/35\\
\pover{\td{3}}{s_1}&=\sum_{i\in\supp{X_{s_1}}=\{1,2,3\}}\p{x,\td{3}}\frac{\pover{X=i}{S=s_1}}{\p{X=i}}=0.1\cdot 0.4/0.7+0.2\cdot 0.5/0.2=39/70,
\end{align*}
such that $P^{\td{X}_{s_1}}=\frac{1}{70}[19,12,39]^{\tr}$. 


The distance that we use is KL divergence.
\begin{definition}[Kullback-Leibler divergence]
Given two discrete measures $a,b$, assuming 
\begin{equation*}
a=\sum_{i}a_i\delta_{x_i},\quad b=\sum_{i}b_i\delta_{x_i}
\end{equation*}
are supported on the same set of $n$ points $(x_i)^n_{i=1}\subset\supp{X}$. Kullback-Leibler divergence is defined as
\begin{equation}
\kl{a}{b}:=\sum_{i\in Supp(b)}a_i\log\left(\frac{a_i}{b_i}\right),
\end{equation}
where $\kl{a}{b}=+\infty$ if $Supp(b)\subset Supp(a)$.
\end{definition}


We estimate the probability mass within $i\in\supp{X}$ by
\begin{equation}
P^{X_s}_i:=\frac{1}{\sigma_{s}\sqrt{2\pi}}\exp^{-\frac{1}{2}\left(\frac{x-\mu_{s}}{\sigma_{s}}\right)^2},
\end{equation}
where $\mu_s$ and $\sigma_s$ are the mean and standard deviation of the variable $X_s$.

\begin{definition}[Source domains]
Let $\supp{X}$ be the support of $\p{x}$ such that
\begin{equation}
\supp{X}:=\{x\in\bb{R}^d\mid\p{x}>0\}.
\end{equation}
It is possible that $\exists x\in\supp{X}$, $\pover{x}{s}=0$, But it holds that $\exists s\in\supp{S}$, $\pover{x}{s}>0$, for all $x\in\supp{X}$.
Further, we define the support of $\pover{x}{s}$:
\begin{equation}
\supp{X}_s:=\{x\in\supp{X}\mid\pover{x}{s}>0\}, \forall s\in\supp{S}.
\end{equation}
\end{definition}

\begin{definition}[Target domain]
Let $\supp{\td{X}}$ be the support of $\p{\tx}$ such that
\begin{equation}
\supp{\td{X}}:=\{\tx\in\bb{R}^d\mid\p{\tx}>0\}.
\end{equation}
It is possible that $\exists \tx\in\supp{\td{X}}$, $\pover{\tx}{s}=0$. But it holds that $\exists s\in\supp{S}$, $\pover{\tx}{s}>0$, for all $\tx\in\supp{\td{X}}$.
\end{definition}



If we restrict $\bbt{X}$ to be the intersection of $\bb{X}_{s_0}$ and $\bb{X}_{s_1}$ and also the region where $\pover{x}{s_0}=\pover{x}{s_1}$, we have total repair guaranteed. To what extend would total repair be violated if $\bbt{X}$ is defined on the subset of $\bb{X}$ where $\pover{x}{s_0}$ and $\pover{x}{s_1}$ are fairly close?

\begin{definition}\label{def:bbt{x}-relax-binary}
Given $\bb{S}=\{s_0,s_1\}$.
Let $\epsilon> 0$.
Let $\bbt{X}^{\epsilon}$ be a subset of $\bb{X}$ such that
\begin{equation}
\bbt{X}^{\epsilon}:=\left\{x\in\bb{X}_{s_0}\bigcap\bb{X}_{s_1}\mid \epsilon/a<\pover{x}{s}\leq\epsilon,\forall s\in\bb{S}\right\}\subseteq\bb{X}.
\end{equation}
From definition, it holds that for $\bbt{X}^{\epsilon}$, $\p{x},\pover{x}{s}\in(\epsilon/a,\epsilon]$ and $|\pover{x}{s_0}-\pover{x}{s_1}|\leq\epsilon(1-1/a)$.
Correspondingly, let 
\begin{equation}
\bb{U}^{\epsilon}:=\left\{\p{x,\tx}\in\mathcal{M}^1_+(\bb{X}\times\bbt{X}^{\epsilon})\mid \sum_{\tx\in\bbt{X}^{\epsilon}}\p{x,\tx}=\p{x},\sum_{x\in\bb{X}}\p{x,\tx}=\p{\tx}\right\}.
\end{equation}
\end{definition}

\begin{lemma}
\begin{proof}
The first equation uses that $\bbt{X}^{\epsilon}\subseteq \bb{X}_{s_0}\bigcap\bb{X}_{s_1}$.
If $\mathbf{P}\in\bb{U}^{\epsilon}$, from definition, it holds that $\p{x,\tx}=0$ for $\p{\tx}\in\bb{X}_{s_0}/\bb{X}_{s_1}$ or $\bb{X}_{s_1}/\bb{X}_{s_0}$.
\begin{align}
\left|\pover{\tx}{s_0}-\pover{\tx}{s_1}\right|&=\sum_{x\in\bb{X}_{s_0}\bigcap\bb{X}_{s_1}}\p{x,\tx}\frac{|\pover{x}{s_0}-\pover{x}{s_1}|}{\p{x}}\\
&\leq\sum_{x\in\bb{X}_{s_0}\bigcap\bb{X}_{s_1}}\p{x,\tx}\frac{|\epsilon(1-1/a)|}{\epsilon/a}\\
&\leq(a-1)\sum_{x\in\bb{X}_{s_0}\bigcap\bb{X}_{s_1}}\p{x,\tx}\\
\end{align}
\end{proof}
\end{lemma}

%\section{Formula for $(X,\td{X},S)$}
\section{Total Repair in general cases}

\begin{theorem}\label{thm:TR-coupling-condition}
Total repair in Definition~\ref{def:total-repair} is achieved, if the coupling $\mathbf{P}\in\bb{U}$ satisfies
\begin{equation}
\sum_{x\in\bb{X}}\p{x,\tx}=\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}},\forall \tx\in\bbt{X},s\in\bb{S}.
\label{equ:coupling-condition}
\end{equation}
Hence, total repair is transformed into a constraint for couplings.
\begin{proof}
Using Lemma~\ref{lem:tx|us},
if one wish to achieve total repair in Definition~\ref{def:total-repair} using this specific coupling $\mathbf{P}\in\bb{U}$, there must exist a probability distribution $\mu^*$ satisfying:
\begin{equation}
\mu^*(\tx)=\pover{x}{s}=\sum_{x\in\bb{X}_s}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}},\;\forall\;s\in\bb{S}.
\end{equation}
Clearly, $\p{\tx}=\mu^*(\tx)$, if $\mu^*(\tx)$ exists.
From the Definition~\ref{def:couplings}, if the coupling $\mathbf{P}\in\bb{U}$ is used, 
\begin{equation}
\mu^*(\tx)=\p{\tx}=\sum_{x\in\bb{X}}\p{x,\tx}.
\end{equation}
Hence,
\begin{equation}
\sum_{x\in\bb{X}}\p{x,\tx}=\sum_{x\in\bb{X}_s}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}.
\end{equation}
\end{proof}
\end{theorem}

\begin{remark}
If $\bb{X}_s=\bb{X}$ and $\pover{x}{s}=\p{x}$, for $x\in\bb{X},s\in\bb{S}$, Equation~\eqref{equ:coupling-condition} is automatically satisfied: any couplings $\mathbf{P}\in\bb{U}$ can project the original dataset $(X,S)$ to $(\td{X},S)$ with total repair guaranteed. If not, one needs to find specific couplings that satisfy Equation~\eqref{equ:coupling-condition} to project the original dataset.
\end{remark}

\section{Our method (need to update)}

Our method starts with a simple trick:

\begin{definition}\label{def:bbt{x}}
Let $\bbt{X}$ be a subset of $\bb{X}$ such that
\begin{equation}
\bbt{X}:=\{x\in\bb{X}\mid \pover{x}{s}=\p{x},\forall s\in\bb{S}\}\subseteq\bb{X}.
\end{equation}
Hence, for arbitrary couplings $\mathbf{P}\in\bb{U}$, it satisfies $\p{x,\tx}=0$ for $x\in\bb{X}/\bbt{X}$ and $\frac{\pover{x}{s}}{\p{x}}= 1$ for $x\in\bbt{X},s\in\bb{S}$. Note that when $\pover{x}{s}=\p{x}$ for $x\in\bb{X},s\in\bb{S}$, $\bbt{X}=\bb{X}$.
\end{definition}

With the definition of $\bbt{X}$ in mind, we recall the constraints in Theorem~\ref{thm:TR-coupling-condition}:


\begin{theorem}
With $\bbt{X}$ being in Definition~\ref{def:bbt{x}}, the total repair in Definition~\ref{def:total-repair} could be satisfied by arbitrary couplings $\mathbf{P}\in\bb{U}$.
\begin{proof}
Given $\p{x,\tx}=0$ for $x\in\bb{X}/\bbt{X}$.
The left part of Equation~\eqref{equ:coupling-condition} can be rewritten as
\begin{equation}
\sum_{x\in\bb{X}}\p{x,\tx}=\sum_{x\in\bb{X}/\bbt{X}}\p{x,\tx}+\sum_{x\in\bbt{X}}\p{x,\tx}=0+\sum_{x\in\bbt{X}}\p{x,\tx}.
\end{equation}
Similarly, the right part of Equation~\eqref{equ:coupling-condition} can be rewritten as
\begin{equation}
\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}=\sum_{x\in\bb{X}/\bbt{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}+\sum_{x\in\bbt{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}=0+\sum_{x\in\bbt{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}.
\end{equation}
Since $\frac{\pover{x}{s}}{\p{x}}= 1$ for $x\in\bbt{X}$, we have that 
\begin{equation}
\sum_{x\in\bbt{X}}\p{x,\tx}=\sum_{x\in\bbt{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}.
\end{equation}
As long as $\bbt{X}$ is defined as in Definition~\ref{def:bbt{x}},
arbitrary couplings $\mathbf{P}\in\bb{U}$ satisfy
Equation~\eqref{equ:coupling-condition} and then we complete the proof.
\end{proof}
\end{theorem}



\subsection{Relaxation}
If we restrict $\bbt{X}$ to be the subset of $\bb{X}$ where $\pover{x}{s_0}=\pover{x}{s_1}$, we have total repair guaranteed. To what extend would total repair be violated if $\bbt{X}$ is defined on the subset of $\bb{X}$ where $\pover{x}{s_0}$ and $\pover{x}{s_1}$ are fairly close? We start from a general setting.

First, we relax the definition of $\bbt{X}$:
\begin{definition}\label{def:bbt{x}-relax}
Let $\epsilon> 0$.
Let $\bbt{X}^{\epsilon}$ be a subset of $\bb{X}$ such that
\begin{equation}
\bbt{X}^{\epsilon}:=\left\{x\in\bb{X}\mid \left|\frac{\pover{x}{s}}{\p{x}}-1\right|\leq\epsilon,\forall s\in\bb{S}\right\}\subseteq\bb{X}.
\end{equation}
When $\epsilon\to 0$, $\bbt{X}^{\epsilon}$ coincides with $\bbt{X}$ in Definition~\ref{def:bbt{x}}, and denote it by $\bbt{X}^0$. Correspondingly, let 
\begin{equation}
\bb{U}^{\epsilon}:=\left\{\p{x,\tx}\in\mathcal{M}^1_+(\bb{X}\times\bbt{X}^{\epsilon})\mid \sum_{\tx\in\bbt{X}}\p{x,\tx}=\p{x},\sum_{x\in\bb{X}}\p{x,\tx}=\p{\tx}\right\}.
\end{equation}
Obviously, $\bbt{X}^0\subseteq\bbt{X}^{\epsilon}$ and $\bb{U}^0\subseteq\bb{U}^{\epsilon}$.
\end{definition}
\textcolor{red}{
The condition for $\bbt{X}^{\epsilon}$: $|\pover{x}{s}-\p{x}|\leq\epsilon\;\p{x}$.\\
A sufficient condition: $\pover{x}{s}\leq a$ and $\p{x}\geq a/\epsilon$, given $\epsilon\geq 1$, $a\in(0,1]$.}

\begin{lemma}\label{lem:violation_TR}
For arbitrary couplings $\mathbf{P}\in\bb{U}^{\epsilon}$, it satisfies $\p{x,\tx}=0$ for $x\in\bb{X}/\bbt{X}^{\epsilon}$ and $\frac{\pover{x}{s}}{\p{x}}= 1$ for $x\in\bbt{X}^{0},s\in\bb{S}$. More importantly, the violation of total repair:
\begin{equation}
\left|\sum_{x\in\bbt{X}}\p{x,\tx}\left(1-\frac{\pover{x}{s}}{\p{x}}\right)\right|\leq\epsilon\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}\leq\epsilon\;\p{\tx},\;\forall\tx\in\bbt{X}^{\epsilon},s\in\bb{S}.
\end{equation}
\begin{proof}
Given a coupling $\mathbf{P}\in\bb{U}^{\epsilon}$, it satisfies $\p{x,\tx}=0$ for $x\in\bb{X}/\bbt{X}^{\epsilon}$.
Now we divide $\bb{X}$ into three subsets: $\bb{X}/\bbt{X}^{\epsilon}$, $\bbt{X}^{\epsilon}/\bbt{X}^0$ and $\bbt{X}^0$.
The left part of Equation~\eqref{equ:coupling-condition} can be rewritten as
\begin{align}
\sum_{x\in\bb{X}}\p{x,\tx}&=\sum_{x\in\bb{X}/\bbt{X}^{\epsilon}}\p{x,\tx}+\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}+\sum_{x\in\bbt{X}^0}\p{x,\tx}\\
&=0+\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}+\sum_{x\in\bbt{X}^0}\p{x,\tx}
\end{align}
The right part of Equation~\eqref{equ:coupling-condition} can be rewritten as
\begin{align}
\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}&=0+\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}+\sum_{x\in\bbt{X}^0}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}
\end{align}
Note that for $x\in\bbt{X}^0,s\in\bb{S}$, $\frac{\pover{x}{s}}{\p{x}}=1$ still holds.
Now, the difference between the left and right side is:
\begin{align}
\sum_{x\in\bb{X}}\p{x,\tx}-\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}&=\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}-\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}\\
&=\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}\left(1-\frac{\pover{x}{s}}{\p{x}}\right).
\end{align}
Due to Definition~\ref{def:bbt{x}-relax}, $\left|\frac{\pover{x}{s}}{\p{x}}-1\right|\leq\epsilon$, such that
\begin{equation}
\left|\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}\left(1-\frac{\pover{x}{s}}{\p{x}}\right)\right|\leq\epsilon\sum_{x\in\bbt{X}^{\epsilon}/\bbt{X}^0}\p{x,\tx}.
\end{equation}
Then, using the fact that $\sum_{x\in\bbt{X}^{\epsilon}}\p{x,\tx}=\p{\tx}$ for $\mathbf{P}\in\bb{U}^{\epsilon}$, we complete the proof.
\end{proof}
\end{lemma}



\begin{lemma}\label{lem:tv_x|s_x}
If $\mathbf{P}\in\bb{U}^{\epsilon}$, the total variation distance between $\pover{\tx}{s}$ and $\p{\tx}$ is less than or equal to $\epsilon/2$.
\begin{proof}
The second equality uses Lemma~\ref{lem:tx|us}. The inequality uses Lemma~\ref{lem:violation_TR}. The last equality utilises the fact that $\sum_{\tx\in\bbt{X}^{\epsilon}} \p{\tx}=1$ for $\mathbf{P}\in\bb{U}^{\epsilon}$.
\begin{align}
\tv{\pover{\tx}{s}}{\p{\tx}}&=\frac{1}{2}\sum_{\tx\in\bbt{X}^{\epsilon}} \left|\pover{\tx}{s}-\p{\tx}\right|\\
&=\frac{1}{2}\sum_{\tx\in\bbt{X}^{\epsilon}} \left|\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}-\sum_{x\in\bb{X}}\p{x,\tx}\right|\\
&\leq\frac{\epsilon}{2}\sum_{\tx\in\bbt{X}^{\epsilon}} \p{\tx}=\frac{\epsilon}{2}.
\end{align}
\end{proof}
\end{lemma}

\begin{lemma}\label{lem:tv_x|s_x|s'}
Let $\bb{S}=\{s_0,s_1,\dots,s_n\}$, $n\geq 1$ and $\mathbf{P}\in\bb{U}^{\epsilon}$. For arbitrary $s_0,s_1\in\bb{S}$, the total variation distance between $\pover{\tx}{s_0}$ and $\pover{\tx}{s_1}$ is less than or equal to $\epsilon$.
\begin{proof}
Using triangle inequalities,
\begin{align}
\left|\pover{\tx}{s_0}-\pover{\tx}{s_1}\right|&=\left|(\pover{\tx}{s_0}-\p{\tx})-(\pover{\tx}{s_1}-\p{\tx})\right|\\
&\leq \left|\pover{\tx}{s_0}-\p{\tx}\right|+\left|\pover{\tx}{s_1}-\p{\tx}\right|.
\end{align}
Using Lemma~\ref{lem:tv_x|s_x},
\begin{align}
\tv{\pover{\tx}{s_0}}{\pover{\tx}{s_1}}&=\frac{1}{2}\sum_{\tx\in\bbt{X}^{\epsilon}} \left|\pover{\tx}{s_0}-\pover{\tx}{s_1}\right|\\
&=\frac{1}{2}\sum_{\tx\in\bbt{X}^{\epsilon}}\left|\pover{\tx}{s_0}-\p{\tx}\right|+\left|\pover{\tx}{s_1}-\p{\tx}\right|\\
&=\frac{1}{2}\sum_{\tx\in\bbt{X}^{\epsilon}}\left|\pover{\tx}{s_0}-\p{\tx}\right|+\frac{1}{2}\sum_{\tx\in\bbt{X}^{\epsilon}}\left|\pover{\tx}{s_1}-\p{\tx}\right|\\
&\leq \epsilon.
\end{align}
\end{proof}
\end{lemma}

So far, we have not yet discussed the target distribution $\p{\tx}$ that has been used in defining $\bb{U}$ and $\bb{U}^{\epsilon}$. In fact, there is no restriction other than $\p{\tx}\in\mathcal{M}^1_+(\bbt{X}^{\epsilon})$. To summarise,

\begin{theorem}\label{thm:summary}
Given $\bbt{X}^{\epsilon}$. Let $\p{\tx}$ be an arbitrary distribution in $\mathcal{M}^1_+(\bbt{X}^{\epsilon})$, we find a set of couplings $\bb{U}^{\epsilon}$.
An arbitrary coupling $\mathbf{P}\in\bb{U}^{\epsilon}$ can transport the original dataset $(X,S)$ to the target dataset $(\td{X},S)$ with 
\begin{align}
\tv{\pover{\tx}{s}}{\p{\tx}}&\leq\frac{\epsilon}{2}, \;\forall s\in\bb{S},\\
\tv{\pover{\tx}{s}}{\pover{\tx}{s'}}&\leq\epsilon,\;\forall s,s'\in\bb{S}.    
\end{align}
\begin{proof}
See Lemma~\ref{lem:tv_x|s_x}-\ref{lem:tv_x|s_x|s'}. Note that in these lemmas, there is no restriction for $\p{\tx}\in\mathcal{M}^1_+(\bbt{X}^{\epsilon})$.
\end{proof}
\end{theorem}

According to Corollary~\ref{cor:binary_condition}, when $\bb{S}=\{s_0,s_1\}$, the situation is much easier.



\section{Existence of target domains}

We know that if $\epsilon$ is sufficiently large, the domain $\bbt{X}^{\epsilon}$ exists.
To ensure the existence of a target domain $\bbt{X}^{\epsilon}$ for a certain $\epsilon>0$, we restrict our attention to sub-Gaussian random variables, which contain Gaussian, Bernoulli and all bounded random variables.

In the following text, we will continuously use $c,C>0$ to denote absolute constants, but please be aware that $c,C$ can be different values throughout the paper, unless specified.

\subsection{Sub-Gaussian random variables (d=1)}

\begin{definition}[Sub-Gaussian random variables; Definition 2.5.5 in \cite{vershynin2018high}]
The random variable $X$, is said to be sub-Gaussian, or $X\sim\sg$, if it satisfies the following equivalent properties (see Proposition 2.5.2 in \cite{vershynin2018high} for the equivalence):
\begin{align}
\p{|X|\geq t}\leq 2\exp(-ct^2/\norm{X}^2)\;,\forall t\geq 0,\label{equ:subG_concentration}\\
\|X\|_p\leq C\norm{X}\sqrt{p}\; ,\forall p\geq 1,\label{equ:norm_lowerbound} \\
\E\exp(X^2/\norm{X}^2)\leq 2.
\end{align}
If $\E X=0$, then for $\lambda\in\bb{R}$
\begin{equation}
\E\exp(\lambda X)\leq\exp(C\lambda^2\norm{X}^2).\label{equ:mean_zero_subG}
\end{equation}
Note that the last property in Equation~\eqref{equ:mean_zero_subG} also imply the three equivalent properties.
The sub-Gaussian norm of $X$, denoted $\norm{X}$, is defined to be
\begin{equation}
\norm{X}:=\inf\{t>0\mid \E\exp(X^2/t^2)\leq 2\}.
\end{equation}
\end{definition}

\begin{remark}[Example 2.5.6 in \cite{vershynin2018high}]
Sub-Gaussian random variables include Gaussian, Bernoulli. More generally, any bounded random variable $X$ is sub-Gaussian with
\begin{equation}
\norm{X}\leq \|X\|_{\infty}/\ln 2. \label{equ:norm_upperbound}
\end{equation}
\end{remark}

\begin{lemma}[Centring; Lemma 2.6.6 in \cite{vershynin2018high}]\label{lem:centring}
If $X$ is a sub-Gaussian random variable, then $X-\E X$ is sub-Gaussian and 
\begin{equation}
\norm{X-\E X}\leq C\norm{X}.
\end{equation}
\begin{proof}
Equations~\eqref{equ:norm_lowerbound} and~\eqref{equ:norm_upperbound}) imply $\norm{\cdot}$ is a norm so triangle inequality yields:
\begin{equation}
\norm{X-\E X}\leq\norm{X}+\norm{\E X}. \label{equ:centering_subG}
\end{equation}
Note that $\E X$ is a constant. Recall the definition of sub-Gaussian norm, we know that $\norm{\E X}=\inf\{t>0:\E\exp((\E X)^2/t^2)\leq2\}$ and
\begin{equation}
\exp\left(\frac{(\E X)^2}{\norm{\E X}^2}\right)=\E\exp\left(\frac{(\E X)^2}{\norm{\E X}^2}\right)\leq2=\exp(\ln 2).
\end{equation}
Since $\norm{\E X}>0$, we obtain $\norm{\E X}\geq|\E X|/\sqrt{\ln 2}$. Further, the first equality utilises that $\norm{\E X}$ is defined to be the minimum that satisfies this property. The first inequality uses Jensen's inequality and the last inequality reuses Equation~\eqref{equ:norm_lowerbound}:
\begin{equation}
\norm{\E X}=|\E X|/\sqrt{\ln 2}\leq\E |X|/\sqrt{\ln 2}=\|X\|_1/\sqrt{\ln 2}\leq c\norm{X}. \label{equ:centering_subG_EX}
\end{equation}
Substituting Equation~\eqref{equ:centering_subG_EX} into \eqref{equ:centering_subG}, we complete the proof.
\end{proof}
\end{lemma}

\begin{lemma}[Sums of independent sub-Gaussians; Proposition 2.6.1 in \cite{vershynin2018high}] \label{lem:sums_of_subG}

Let $X_1,\dots,X_n$ be independent, mean zero, sub-Gaussian random variables. Then $\sum_{i=1}^n X_i$ is also a sub-Gaussian random variable and
\begin{equation}
\norm{\sum_{i=1}^n X_i}^2\leq C\sum_{i=1}^n \norm{X_i}^2.
\end{equation}
\begin{proof}
For any $\lambda\in\bb{R}$, we have the following formula. The first equality uses the independence between $X_1,\dots,X_n$. The second inequality utilises $X_1,\dots,X_n$ are mean zero, sub-Gaussian and Equation~\eqref{equ:mean_zero_subG}.
\begin{align}
\E\exp(\lambda\sum_{i=1}^n X_i)=\prod_{i=1}^n\E\exp(\lambda X_i)\leq\prod_{i=1}^n\exp(c\lambda^2\norm{X_i}^2)=\exp(c\lambda^2\sum_{i=1}^n\norm{X_i}^2).
\end{align}
The above formula show that $\sum_{i=1}^n X_i$ is also sub-Gaussian by satisfying the property in Equation~\eqref{equ:mean_zero_subG}.
\end{proof}
\end{lemma}

\begin{remark}[Expectation of a linear combination]\label{rem:expectation_X}
Under Assumption~\ref{ass:independent_subG},
\begin{equation}
\E X=\E \sum_{s\in\bb{S}}X_s\p{s}= \sum_{s\in\bb{S}}\p{s}\E X_s.
\end{equation}
\end{remark}

\subsection{A subset of the relaxed target domain}
\begin{definition}
For $s\in\bb{S}$, let $X_s\in\bb{X}$ be a random variables such that $\p{X_s=x}:=\pover{x}{s}$. Let $X\in\bb{X}$ be a random variable that 
\begin{equation}
X=\sum_{s\in\bb{S}}X_s \p{s}.
\end{equation}
\end{definition}

\begin{assumption}[$X_s$ is sub-Gaussian]\label{ass:independent_subG}
For $s\in\bb{S}$, let $X_s$ be a one-dimensional sub-Gaussian random variable with mean $\E X_s$ and centring sub-Gaussian norm $\norm{X_s-\E X_s}$. Using Lemma~\ref{lem:centring}, $\norm{X_s-\E X_s}\leq C\norm{X_s}$.
Further, assume $X_s$ for $s\in\bb{S}$ are independent sub-Gaussians. 
\end{assumption}

Now, we will show that $X$ is also sub-Gaussian, following Lemma~\ref{lem:sums_of_subG}.

\begin{lemma}[$X-\E X$ is sub-Gaussian]\label{lem:X-EX_subG}
Under Assumption~\ref{ass:independent_subG}, $X-\E X$ is also sub-Gaussian, with the square of its sub-Gaussian norm:
\begin{equation}
\norm{X-\E X}^2\leq C\sum_{s\in\bb{S}}\norm{X_s-\E X_s}^2 \p{s}^2.\label{equ:square_subG_norm}
\end{equation}
\begin{proof}
For any $\lambda\in\bb{R}$, we have the following formula. 
The first equality uses Remark~\ref{rem:expectation_X}.
The third equality uses the independence between $X_s$ for $s\in\bb{S}$. 
The first inequality utilises $X_s$ is mean zero, sub-Gaussian with $\norm{X_s-\E X_s}$ and Equation~\eqref{equ:mean_zero_subG}.
\begin{align}
\E\exp(\lambda( X-\E X))
&=\E\exp\left(\lambda\sum_{s\in\bb{S}} \p{s}\left(X_s-\E X_s\right)\right)=\E\exp\left(\sum_{s\in\bb{S}} \lambda\p{s}\left( X_s-\E X_s\right)\right)\\
&=\prod_{s\in\bb{S}}\E\exp\left( \lambda\p{s}\left( X_s-\E X_s\right)\right)\\
&\leq\prod_{s\in\bb{S}}\exp(c\lambda^2\p{s}^2\norm{X_s-\E X_s}^2)\\
&=\exp(c\lambda^2\sum_{s\in\bb{S}}\p{s}^2\norm{X_s-\E X_s}^2).
\end{align}
The above formula show that $X-\E X$ is also sub-Gaussian, with the square of sub-Gaussian norm satisfying Equation~\eqref{equ:square_subG_norm}. 
\end{proof}
\end{lemma}

\begin{lemma}[Concentration inequalities]\label{lem:concentration_inequalities}
Under Assumption~\ref{ass:independent_subG}, we have the following concentration inequalities for all $t\geq 0$:
\begin{align}
\p{|X_s-\E X_s|\geq t}&\leq 2\exp(-t^2/\norm{X_s-\E X_s}^2),\\
\p{|X\;-\E X\;|\geq t}&\leq 2\exp\left(-
\frac{C\;t^2}{\sum_{s\in\bb{S}}\norm{X_s-\E X_s}^2 \p{s}^2}\right).\label{equ:concentration_inequalities}
\end{align}
\begin{proof}
Both inequalities follow the sub-Gaussian property in Equation~\eqref{equ:subG_concentration}, with unknown absolute constants.
However, to find the value of these absolute constant, we apply Markov's inequality:
\begin{align}
\p{|X_s-\E X_s|\geq t}&=\p{\frac{(X_s-\E X_s)^2}{\norm{X_s-\E X_s}^2}\geq \frac{t^2}{\norm{X_s-\E X_s}^2}}\\
&=\p{\exp\frac{(X_s-\E X_s)^2}{\norm{X_s-\E X_s}^2}\geq \exp\frac{t^2}{\norm{X_s-\E X_s}^2}}\\
&\leq\exp\left(-\frac{t^2}{\norm{X_s-\E X_s}^2}\right)\E \exp\left(\frac{(X_s-\E X_s)^2}{\norm{X_s-\E X_s}^2}\right)\\
&\leq 2\exp\left(-\frac{t^2}{\norm{X_s-\E X_s}^2}\right),
\end{align}
such that the absolute constant in Equation~\eqref{equ:subG_concentration} is $1$. Further, Equation~\eqref{equ:concentration_inequalities} also utilises Lemma~\ref{lem:X-EX_subG}:
\begin{equation}
\p{|X-\E X|\geq t}\leq 2\exp(-t^2/
\norm{X-\E X}^2)\leq 2\exp\left(-
\frac{C\;t^2}{\sum_{s\in\bb{S}}\norm{X_s-\E X_s}^2 \p{s}^2}\right).
\end{equation}
\end{proof}
\end{lemma}

\begin{lemma}\label{lem:x^a}
Given a constant $a\in(0,1]$. Under Assumption~\ref{ass:independent_subG}, we show that 
\begin{equation}
\pover{x}{s}\leq a,\forall x\in\bb{X}^a,s\in\bb{S}, 
\end{equation}
where
\begin{align}
\bb{X}^a:&=\bb{X}/\bigcup_{s\in\bb{S}}(\E X_s -t_s,\E X_s +t_s),\\
t_s:&=\sqrt{\ln{(2/a)}}\norm{X_s-\E X_s}. %=\sqrt{-\ln{(a/2)}\;\min_{s\in\bb{S}}\norm{X_s-\E X_s}^2}
\end{align}
\begin{proof}
Under Assumption~\ref{ass:independent_subG} and using Lemma~\ref{lem:concentration_inequalities}, the definition of $t_s$ implies that for all $s\in\bb{S}$:
\begin{align}
\p{|X_s-\E X_s|\geq t_s}&\leq 2\exp(-(t_s)^2/\norm{X_s-\E X_s}^2)\\
&=2\exp\left(\ln{(a/2)}\norm{X_s-\E X_s}^2/\norm{X_s-\E X_s}^2\right)=a,
\end{align}
Hence, it follows: 
\begin{align}
\sum_{x\in\bigcup_{s\in\bb{S}}(\E X_s-t_s, \E X_s+t_s)}\pover{x}{s}&\geq\sum_{x\in(\E X_s-t_s, \E X_s+t_s)}\pover{x}{s}\\
&=\p{|X_s-\E X_s|< t_s}\\
&=1-\p{|X_s-\E X_s|\geq t_s}\\
&\geq 1-a.
\end{align}
Further, since $\sum_{x\in\bb{X}}\pover{x}{s}=1$, it holds that for any $x\in\bb{X}/\bb{X}^a$,
\begin{align}
\pover{x}{s}\leq\sum_{x\in\bb{X}/\bb{X}^a}\pover{x}{s}=1-\sum_{x\in\bb{X}^a}\pover{x}{s}\leq a.
\end{align}
Note that for $x\in\bb{X}^a$, it also holds that $\p{x}\leq a$.
\end{proof}
\end{lemma}

Intuitively, when $a$ is small, the subset $\bb{X}^a$ is at the tails of two sides of distributions of all $X_s$, $s\in\bb{S}$. Since $X$ is also sub-Gaussian, the region where $\p{x}\geq a/\epsilon$ holds should be in the middle of the distribution of $X$. On the intersection of the tails in $\bb{X}^a$ and the middle of the distribution of $X$, we might find a subset of $\bbt{X}^{\epsilon}$ in Definition~\ref{def:bbt{x}}.
However, with the concentration inequalities for $X$, we are not able to specify the region where $\p{x}\geq a/\epsilon$ always holds.


\begin{theorem}
Given an $\epsilon\geq 1$ and a constant $a\in(0,1]$. Under Assumption~\ref{ass:independent_subG}, we define
\begin{equation}
\bb{X}^{a}_{a/\epsilon}:=\{x\in\bb{X}\mid \p{x}\geq a/\epsilon\}\bigcap\bb{X}^{a},\label{equ:X^a_{a/e}}
\end{equation}
such that $\bb{X}^{a}_{a/\epsilon}\subseteq\bbt{X}^{\epsilon
}$. Further, let $\p{\tx}$ be an arbitrary distribution in $\mathcal{M}^1_+(\bb{X}^{a}_{a/\epsilon})$, we find a set of couplings $\bb{U}^{\epsilon}$.
An arbitrary coupling $\mathbf{P}\in\bb{U}^{\epsilon}$ can transport the original dataset $(X,S)$ to the target dataset $(\td{X},S)$ with 
\begin{align}
\tv{\pover{\tx}{s}}{\p{\tx}}&\leq\frac{\epsilon}{2}, \;\forall s\in\bb{S},\\
\tv{\pover{\tx}{s}}{\pover{\tx}{s'}}&\leq\epsilon,\;\forall s,s'\in\bb{S}.    
\end{align}
\begin{proof}
Using Lemma~\ref{lem:x^a}, it holds that $\pover{x}{s}\leq a$ for $x\in\bb{X}^a$, $s\in\bb{S}$. Hence, Equation~\eqref{equ:X^a_{a/e}} implies that
\begin{equation}
\p{x}\geq a/\epsilon \textrm{ and } \pover{x}{s}\leq a,\forall x\in \bb{X}^{a}_{a/\epsilon},s\in\bb{S}.
\end{equation}
Firstly, since $\pover{x}{s}\leq a$ for $s\in\bb{S}$, 
\begin{equation}
\p{x}=\sum_{s\in\bb{S}}\pover{x}{s}\p{s}\leq a\sum_{s\in\bb{S}}\p{s}=a.
\end{equation}
Then since $\p{x},\pover{x}{s}\leq a$ and $\p{x}\geq a/\epsilon$, we know that
\begin{equation}
\left|\frac{\pover{x}{s}}{\p{x}}-1\right|=\frac{\left|\pover{x}{s}-\p{x}\right|}{\p{x}}\leq\frac{a}{\p{x}}\leq\frac{a}{a/\epsilon}=\epsilon.
\end{equation}
Hence, we conclude that $\bb{X}^{a}_{a/\epsilon}\subseteq\bbt{X}^{\epsilon}$.
Further, reuse Theorem~\ref{thm:summary}, we complete the proof.
\end{proof}
\end{theorem}

\begin{corollary}
When $\bb{S}=\{s_0,s_\}$, the subset could be
\end{corollary}

\section{Shape constraints for target distributions}
Theorem~\ref{thm:summary} provides a solution to total repair when the target distribution belongs to $\mathcal{M}^1_+(\bbt{X}^{\epsilon})$. However, 
there could be shape constraints for the ultimate target distribution $\p{x^*}$, for instance, $\p{x^*}\in\mathcal{M}^1_+(\bb{X}^*)$ while $\bbt{X}^{\epsilon}\subset\bb{X}^*$, $\bbt{X}^{\epsilon}\cap\bb{X}^*=\emptyset$ or more generally $\bb{X}^*\in\bb{R}^d$.
To do so, we first transport $\p{x}$ to $\p{\tx}\in\mathcal{M}^1_+(\bbt{X}^{\epsilon})$ and then transport $\p{\tx}$ to $\p{x^*}\in\mathcal{M}^1_+(\bb{X}^*)$.
Under certain assumptions, we can limit the distance within a specific range.

\begin{align}
\bb{X}&:=[0,10]\\
\bbt{X}&:=[5,10]\subset\bb{X}\\
\bb{X}^*&:=[20,30]\subset\bb{R}
\end{align}
We design 
\begin{equation}
\p{2\tx+10}:=\p{x^*}
\end{equation}

%$\min\tv{\p{\tx}}{\p{x}}$ while $\bbt{X}^{\epsilon}\subset\bb{X}$. In this case, $\tv{\p{\tx}}{\p{x}}\neq 0$ but under certain assumptions, we can limit the distance within a specific range.




\begin{lemma}\label{lem:tx|us}
If one wish to achieve total repair in Definition~\ref{def:total-repair} using this specific coupling $\p{x,\tx}\in\bb{U}$, there must exist a probability distribution $\mu^*$ satisfying:
\begin{equation}
\mu^*(\tx)=\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}},\;\forall\;s\in\bb{S}.
\end{equation}
\begin{proof}
Using Lemma~\ref{lem:T2Ts},
\begin{equation}
\pover{\tx}{s}=\frac{\p{\tx,s}}{\p{s}}=\frac{\sum_{x\in\bb{X}}\p{x,\tx,s}}{\p{s}}=\frac{\sum_{x\in\bb{X}}\p{x,\tx}\pover{s}{x}}{\p{s}}.
\end{equation}
Since
\begin{equation}
\frac{\pover{s}{x}}{\p{s}}=\frac{\p{s,x}}{\p{x}\p{s}}=\frac{\pover{x}{s}}{\p{x}},
\end{equation}
we can rewrite
\begin{equation}
\pover{\tx}{s}=\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{s}{x}}{\p{s}}=\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}.
\end{equation}
\end{proof}
\end{lemma}

\begin{remark}\label{rem:tx|u=mu*}
Clearly, $\p{\tx}=\mu^*(\tx)$, if $\mu^*(\tx)$ exists.
\end{remark}


\begin{assumption}
\begin{equation}
\p{s}>0,\;\pover{x}{s}>0, \forall x\in\bb{X},  s\in\bb{S}.
\end{equation}
Hence, $\p{x,s}>0$ and $\pover{\tx}{x,s}$ exists for $x\in\bb{X}$ and $s\in\bb{S}$.
\end{assumption}

\begin{lemma}\label{rem:xhat_ij=xhat_i}
Since the projection $T$ from $X$ to $\td{X}$ is irrelevant to $S$,
\begin{equation}
\pover{\tx}{x,s}=\pover{\tx}{x}.
\end{equation}
\end{lemma}

\begin{lemma}\label{lem:T2Ts}
When the coupling $\p{x,\tx}\in\bb{U}$ is implemented to transport samples $(X,S)$, it is equivalent to using sub-couplings $\p{x,\tx,s}$ to transport samples $(X,S=s)$, respectively: 
\begin{equation}
\p{x,\tx,s}=\p{x,\tx}\pover{s}{x}.
\end{equation}
\begin{proof} Using Bayesian's theorem,
\begin{align}
\pover{\tx}{x,s}&=\frac{\p{x,\tx,s}}{\p{x,s}},\\
\pover{\tx}{x}&=\frac{\p{x,\tx}}{\p{x}}.
\end{align}
Using Lemma~\ref{rem:xhat_ij=xhat_i},
\begin{equation}
\p{x,\tx,s}=\p{x,\tx}\frac{\p{x,s}}{\p{x}}=\p{x,\tx}\pover{s}{x}.
\end{equation}
\end{proof}
\end{lemma}


Similarly, we define the $S$-conditional coupling $\pover{x,\tx}{s}\geq 0$, such that
\begin{equation}
\sum_{\tx\in\bbt{X}}\pover{x,\tx}{s}=\pover{x}{s},\quad
\sum_{x\in\bb{X}}\pover{x,\tx}{s}=\pover{\tx}{s},\quad \forall\;s\in\bb{S}.
\end{equation}


\begin{remark}
\begin{equation}
\p{\tx}=\sum_{x\in\bb{X}}\pover{\tx}{x}\cdot\p{x}.
\end{equation}
\begin{proof}
Using couplings in Definition~\ref{def:couplings},
\begin{equation}
\p{\tx}=\sum_{x\in\bb{X}}\p{x,\tx}=\sum_{x\in\bb{X}}\frac{\p{x,\tx}}{\p{x}}\p{x}=\sum_{x\in\bb{X}}\pover{\tx}{x}\cdot\p{x}.
\end{equation}
\end{proof}
\end{remark}

\begin{definition}[The feasibility problem]
If the formulation below has at least one feasible solution, there exist $U$-conditional couplings that can make total repair possible.
\begin{align*}
\min_{\p{x,\tx}}& 1\\
s.t.& \sum_{x\in\bb{X}}\p{x,\tx}=\sum_{x\in\bb{X}}\p{x,\tx}\frac{\pover{x}{s}}{\p{x}}\; \forall\tx\in\bbt{X},s\in\bb{S},\\
&\sum_{\tx\in\bbt{X}}\p{x,\tx}=\p{x}\; \forall x\in\bb{X},\\
& 0\leq\p{x,\tx}\leq 1\; \forall x\in\bb{X}, \tx\in\bbt{X}.
\end{align*}
\end{definition}


Given projected dataset $(\tx,u_n,w_{n,\tx})_{\tx\in\bbt{X},n=1,\dots,N}$.
The sample set can be reorganised into $(\tx,u,w_{x,u})_{x\in\bb{X},u\in\bb{U}}$, where
\begin{align}
w_{x,u}=\sum^N_{n=1} \mathds{1}_{\{x_n=x\}\wedge\{u_n=u\}}.
\end{align}
In other words, the weight $w_{x,u}$ is the count of samples satisfying $x_n=x$ and $u_n=u$.
Even thought $S$ is unobservant, in the following implementation, we need it for verification purposes. We propose another organisation of dataset: the sample set $(x_n,u_n,s_n)^{N}_{n=1}$ are organised into $(x,u,s,w_{x,u,s})_{x\in\bb{X},u\in\bb{U},s\in\bb{S}}$, where
\begin{align}
w_{x,u,s}=\sum^N_{n=1} \mathds{1}_{\{x_n=x\}\wedge\{u_n=u\}\wedge\{s_n=s\}}.
\end{align}
In other words, the weight $w_{x,u,s}$ is the count of sample $(x,u,s)$. Note that $\sum_{s\in\bb{S}}w_{x,u,s}=w_{x,u}$.
\end{definition}

\begin{remark}
\begin{align}
\kl{x|u,s}{x|u}&:=\sum_{x\in\bb{X}} \pover{x}{u,s}\ln\left(\frac{\pover{x}{u,s}}{\pover{x}{u}}\right)\\
&=\sum_{x\in\bb{X}} \pover{x}{u,s}\ln\left(\frac{\pover{s}{x,u}}{\pover{s}{u}}\right)\\
&=\sum_{x\in\bb{X}} \pover{x}{u,s}\ln\left(\pover{s}{x,u}\right)-\ln\left(\pover{s}{u}\right)\cdot\sum_{x\in\bb{X}}\pover{x}{u}\\
&=\sum_{x\in\bb{X}} \pover{x}{u,s}\ln\left(\pover{s}{x,u}\right)-\ln\left(\pover{s}{u}\right).
\end{align}
\end{remark}

\begin{lemma}\label{lem:Xhat=y_X=z}
Corresponding to $\gamma_u$, 
\begin{equation}
\sum_{x\in\bb{X}}\left(x,u,w\cdot\pover{\tx}{x,u}\right)=T^{-1}(\tx,u,w).
\end{equation}
Note that $\sum_{x\in\bb{X}}\pover{\tx}{x,u}$ does not necessarily equal to $1$.
\begin{proof}
Using couplings in Definition~\ref{def:couplings},
\begin{equation}
\pover{\tx}{u}=\sum_{x\in\bb{X}}\pover{x,\tx}{u}=\sum_{x\in\bb{X}}\frac{\pover{x,\tx}{u}}{\pover{x}{u}}\pover{x}{u}=\sum_{x\in\bb{X}}\pover{\tx}{x,u}\cdot \pover{x}{u},
\end{equation}
\end{proof}
\end{lemma}

\section{Formula for $(X,U,S)$}
\begin{lemma}\label{lem:X|US_X|U}
%The divergence between $\pover{x}{u,s}$ and $\pover{x}{u}$ are related to $\pover{s}{x,u}$ and $\pover{s}{u}$.
\begin{equation}
\pover{x}{u,s}=\frac{\pover{s}{x,u}}{\pover{s}{u}}\pover{x}{u},\quad\forall\; u\in\bb{U}, s\in\bb{S}.
\end{equation}
\begin{proof} For any $x\in\bb{X},u\in\bb{U}$ and $s\in\bb{S}$, we have
\begin{align}
\pover{x}{u,s}&=\frac{\p{x,u,s}}{\p{u,s}}=\frac{\pover{s}{x,u}\p{x,u}}{\p{u,s}},\\
&=\frac{\pover{s}{x,u}\pover{x}{u}\p{u}}{\pover{s}{u}\p{u}}.
\end{align}
\end{proof}
\end{lemma}

\section{Formula for $(\td{X},U,S)$}
\begin{remark}
\begin{align}
\kl{\tx|u,s}{\td{x}|u}&=\sum_{\tx\in\bbt{X}} \pover{\tx}{u,s}\ln\left(\frac{\pover{\tx}{u,s}}{\pover{\tx}{u}}\right)=0, \forall\;u\in\bb{U}, s\in\bb{S}.\\
\kl{\tx|u,s}{x|u}&=\kl{\tx|u}{x|u}\\
\kl{\tx|u,s}{X|u,s}&=\kl{\tx|u}{X|u,s}
\end{align}
\end{remark}

\begin{remark}
\begin{equation}
\pover{s}{\tx,u}=\pover{s}{u},\quad\forall \tx\in\bbt{X}, u\in\bb{U}, s\in\bb{S}.
\end{equation}
\begin{proof}
Lemma~\ref{lem:X|US_X|U} also applies to the target dataset $(\Tilde{X},U,S)$, and Remark~\ref{rem:independence}, thus
\begin{equation}
\pover{\tx}{u,s}=\frac{\pover{s}{\tx,u}}{\pover{s}{u}}\pover{\tx}{u}=\frac{\pover{s}{\tx,u}}{\pover{s}{u}}\pover{\tx}{u,s}.
\end{equation}
\end{proof}
\end{remark}

\begin{align}
\kl{\tx|u}{x|u,s}
&:=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u}\ln\left(\frac{\pover{\tx}{u}}{\pover{x}{u,s}}\right)\\
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u}\ln\left(\frac{\pover{\tx}{u}}{\pover{x}{u}}\cdot\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)\\
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u}\ln\left(\frac{\pover{\tx}{u}}{\pover{x}{u}}\right)+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u}\ln\left(\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)\\
&=\kl{\tx|u}{x|u}+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u}\ln\left(\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)\\
&=\kl{\tx|u}{x|u} +\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{x}{u}\ln\left(\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)\\
&\quad+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \left(\pover{\tx}{u}-\pover{x}{u}\right)\ln\left(\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)\\
%%
&=\kl{\tx|u}{x|u}+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{x}{u}\ln\left(\frac{\pover{x}{u}}{\pover{x}{u,s}}\right)\\
&\quad+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \left(\pover{\tx}{u}-\pover{x}{u}\right)\ln\left(\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)\\
&=\kl{\tx|u}{x|u}+\kl{x|u}{X|u,s}+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \left(\pover{\tx}{u}-\pover{x}{u}\right)\ln\left(\frac{\pover{s}{u}}{\pover{s}{x,u}}\right)
\end{align}

\begin{align}
\pover{s}{\tx,u}&=\frac{\pover{\tx}{u,s}\pover{s}{u}}{\pover{\tx}{u}}\\
&=\frac{\pover{\tx}{u,s}\pover{s}{u}}{\sum_{x\in\bb{X}}\pover{\tx}{x,u}\cdot \pover{x}{u}}
\end{align}

\begin{align}
\kl{\tx|u,s}{x|u}&:=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u,s}\ln\left(\frac{\pover{\tx}{u,s}}{\pover{x}{u}}\right)\\
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u,s}\ln\left(\frac{\pover{\tx}{u,s}}{\pover{\tx}{u}}\frac{\pover{\tx}{u}}{\pover{x}{u}}\right)\\
%&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u,s}\ln\left(\frac{\pover{s}{\tx,u}}{\pover{s}{u}}\frac{\pover{\tx}{u}}{\pover{x}{u}}\right)\\
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u,s}\ln\left(\frac{\pover{\tx}{u,s}}{\pover{\tx}{u}}\right)+\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \pover{\tx}{u,s}\ln\left(\frac{\pover{\tx}{u}}{\pover{x}{u}}\right)\\
&=\kl{\tx|u,s}{\td{x}|u}+\kl{\tx|u}{x|u}
\end{align}

\begin{align*}
\kl{x}{\td{x}}&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}}  \p{x}\ln\left(\frac{\p{x}}{\p{\tx}}\right)\\
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \sum_{u\in\bb{U}} \p{x,u}\ln\left(\frac{\p{x,u}}{\p{\tx,u}}\right)
=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \sum_{u\in\bb{U}}\p{u}\pover{x}{u}\ln\left(\frac{\pover{x}{u}}{\pover{\tx}{u}}\right)
\\
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \mathop{\sum}_{u\in\bb{U}\atop s\in\bb{S}} \p{x,u,s}\ln\left(\frac{\p{x,u,s}}{\p{\tx,u,s}}\right)
=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}} \mathop{\sum}_{u\in\bb{U}\atop s\in\bb{S}}\p{u,s}\pover{x}{u,s}\ln\left(\frac{\pover{x}{u,s}}{\pover{\tx}{u,s}}\right)\\
\kl{x|u}{\td{x}|u}
&=\mathop{\sum}_{x=\tx,\atop x\in\bb{X},\tx\in\bbt{X}}\pover{x}{u}\ln\left(\frac{\pover{x}{u}}{\pover{\tx}{u}}\right)
\end{align*}

Notice that
\begin{equation}
\sum_{x\in\bb{X}}\pover{x,\tx}{u}=\sum_{x\in\bb{X}}\hpover{x,\tx}{u,s=0}=\sum_{x\in\bb{X}}\hpover{x,\tx}{u,s=1}=\mu.
\end{equation}
Meanwhile,
\begin{equation}
\sum_{s\in\bb{S}}\sum_{\tx\in\bbt{X}}\hpover{x,\tx}{u,s}\pover{u}{s}=\sum_{s\in\bb{S}}\pover{x}{u,s}\pover{u}{s}=\pover{x}{u}=\sum_{\tx\in\bbt{X}}\pover{x,\tx}{u},
\end{equation}
such that 
\begin{equation}
\pover{u}{s=0}\sum_{\tx\in\bbt{X}}\hpover{x,\tx}{u,s=0}+\pover{u}{s=1}\sum_{\tx\in\bbt{X}}\hpover{x,\tx}{u,s=1}=\sum_{\tx\in\bbt{X}}\pover{x,\tx}{u},
\end{equation}

\begin{lemma}
Assume there is a solution satisfying Definition~\ref{def:problem-1}, such that there exists $\hpover{\tx}{u,s=0}=\hpover{\tx}{u,s=1}$. We already know $\hpover{\tx}{u}=\mu$, hence
\begin{equation}
\hpover{\tx}{u,s=0}=\hpover{\tx}{u,s=1}=\hpover{\tx}{u}=\mu.
\end{equation}

%Notice that both $\hpover{\tx}{u,s=0}$ and $\hpover{\tx}{u,s=1}$ are achieved by the single coupling $\pover{x,\tx}{u}$, such that
Using $\pover{x}{u,s=0}$ and the computed $\hpover{\tx}{u,s=0}$, we can find possibly many coupling $\gamma_{u,s=0}(x,\tx)$ between $\pover{x}{u,s=0}$ and $\hpover{\tx}{u,s=0}$, denoted by a set
\begin{equation}
\Gamma_{s=0}:=\left\{ \gamma_{u,s=0}(x,\tx) \;\bigl\vert\;\sum_{\tx\in\bbt{X}}\gamma_{u,s=0}(x,\tx)=\pover{x}{u,s=0},\sum_{x\in\bb{X}}\gamma_{u,s=0}(x,\tx)=\mu\right\}.
\label{equ:requirement-1}
\end{equation}
Similarly, for the $s=1$, we can find possibly many coupling $\gamma_{u,s=1}(x,\tx)$ between $\pover{x}{u,s=1}$ and $\hpover{\tx}{u,s=1}$, denoted by a set
\begin{equation}
\Gamma_{s=1}:=\left\{ \gamma_{u,s=1}(x,\tx) \;\bigl\vert\;\sum_{\tx\in\bbt{X}}\gamma_{u,s=1}(x,\tx)=\pover{x}{u,s=1},\sum_{x\in\bb{X}}\gamma_{u,s=1}(x,\tx)=\mu\right\}.
\label{equ:requirement-2}
\end{equation}
Notice that
\begin{equation}
\hpover{x,\tx}{u,s=0}\in\Gamma_{s=0},\quad\hpover{x,\tx}{u,s=1}\in\Gamma_{s=1}.
\end{equation}
Hence
\begin{equation}
\hpover{x}{u,s}=\mu=\sum_{x\in\bb{X}}\pover{x,\tx}{u}\frac{\pover{x}{u,s}}{\pover{x}{u}}, \forall\; s\in\bb{S}.\label{eqU:impossibility-2}
\end{equation}
\textcolor{red}{If $\pover{x}{u,s}\neq\pover{x}{u}$, $\hpover{x,\tx}{u,s=0}\neq\hpover{x,\tx}{u,s=1}$}, this is in conflict with Equation~\eqref{eqU:impossibility-2}.
\end{lemma}

